Polynomial-time Sparse Measure Recovery: From Mean Field Theory to Algorithm Design

Mean field theory has provided theoretical insights into various algorithms by letting the problem size tend to infinity. We argue that the applications of mean-field theory go beyond theoretical insights as it can inspire the design of practical algorithms. Leveraging mean-field analyses in physics, we propose a novel algorithm for sparse measure recovery. For sparse measures over $\mathbb{R}$, we propose a polynomial-time recovery method from Fourier moments that improves upon convex relaxation methods in a specific parameter regime; then, we demonstrate the application of our results for the optimization of particular two-dimensional, single-layer neural networks in realizable settings.

==> backup.tex <==
\subsection{Recovery with an energy distance minimization}
Consider the empirical measure $\mu_n := \frac{1}{n} \sum_{i=1}^n \delta_{w_i}$ where $w_i$ is a $d$-dimensional vector with coordinates $[w_{i}]_1,\dots, [w_i]_d \in [0,\pi]$. Our goal is the recovery of measure $\mu_n$ by minimizing the following energy distance: 
\begin{align}
    n^2 \text{E}_{V} \left(\frac{1}{n} \sum_{i=1}^n \delta_{v_i},\frac{1}{n} \sum_{i=1}^n \delta_{w_i} \right) = \sum_{i,j=1}^n V(v_i - v_j) -  2 \sum_{i,j=1}^n V(w_i - v_j) + \sum_{i,j=1}^n V(w_i - w_j)
\end{align}
We design a particular V to recover $\mu_n$. In particular, we use
\begin{align}
    V_\alpha^q(\Delta) = \sqrt{\alpha_1 [\Delta]_1^2 + \alpha_2 [\Delta]_q^2}
\end{align}
where $\alpha \in \R_+^2$ is a parameter used in the recovery algorithm. The proposed recovery method is a coordinate descent method on E$_{V_\alpha^q}$ for two choices of $\alpha$ and $q$. Algorithm~\ref{alg:recovery_2d} represents the recovery method whose convergence is established in the next lemma.
\begin{algorithm}[h!]
\caption{$d$-dimensional measure recovery}\label{alg:recovery_d}
\begin{algorithmic}
\Require Constants $\beta,\epsilon\in \R^+$, and $\frac{\partial \text{E}_{V_{\alpha}^q}}{\partial [v_{i}]_q}$. 
\State $K=\floor{\sqrt{d}n^2\pi^2/\epsilon}+1 , H=4n\sqrt{d} \log(1/\epsilon)/\epsilon+K, \gamma_1= \epsilon/(4\beta\sqrt{d}),\gamma_2= \epsilon n^2/(2\sqrt{d})$.
\For{$j=1,\dots, K$}
\State $\alpha = (1,0)$
  \State $[v_{i}^{(j+1)}]_1 = [v_{i}^{(j)}]_1 -\left( \frac{\gamma_1}{n^2 \pi}\right) \frac{\partial \text{E}_{V_{\alpha}^1}}{\partial [v_{i}]_1}\mid_{v^{(j)}}$
\EndFor
\For{$j=K+1,\dots,H$}
\For{$q=2,\dots, d$}
\For{$i=1,\dots, n$}
  \State  $\alpha = (\beta,1)$
  \State $[v_{i}^{(j+1)}]_q = [v_{i}^{(j)}]_q -\left( \frac{\gamma_2}{n^2 \pi}\right) \frac{\partial \text{E}_{V_{\alpha}^q}}{\partial [v_{i}]_q}\mid_{v^{(j)}}$
\EndFor
\EndFor
\EndFor
\vspace{0.2cm}
 
\State \textbf{Return} $v_1^{(H)},\dots, v_{n}^{(H)}$
\end{algorithmic}
\end{algorithm}

\begin{lemma}
Suppose that $\Delta(w) := \min_{q \in [n]}\min_{i\neq j} |[w_i]_q-[w_j]_q|>0$. Algorithm~\ref{alg:recovery_2d} with parameters $\beta = 4n^2/\Delta(w)^2$, and $\epsilon<\Delta(w)/2$ yields 
\begin{align}
    \min_{\sigma \in \Lambda} \max_i \| v^{(H)}_i - w_{\sigma(i)}\| \leq \epsilon
\end{align}
where $\Lambda$ contains all the permutations of indices $\{1,\dots, n\}$. Furthermore, the total iteration complexity of this algorithm is \[\bigo\left(\frac{n^4 d^{3/2}\log(1/\epsilon)}{(\Delta(w))^2 \epsilon}\right). \]
\end{lemma}
\begin{proof}
According to Lemma~\ref{lemma:gd_convergence}, there exists a permutation $\sigma$ such that
\begin{align} \label{eq:optimality_1st}
    \left| \left[v_{i}^{(K)}\right]_1 - [w_{\sigma(i)}]_1 \right| \leq \epsilon_1, \quad \quad \epsilon_1 := \min\left\{\frac{\epsilon}{2\sqrt{d}}, \frac{1}{2\beta} \right\}
\end{align}
holds for $K = \floor{\sqrt{d}\pi^2n^2/\gamma_1}+1$. Therefore, the first coordinate of each $w_i$ is recovered in the first phase of optimization when $j\leq K$. This allows the recovery of the rest of the coordinates, since the gradient for parameter choice $(\beta,1)$ (used after $K$ steps) admits a particular structure. 
\begin{align}
    (0.5 n^2) \left( \frac{\partial \text{E}_{V_\alpha^q}}{[\partial v_i]_q} \right)= \sum_{j} \left( c_q(v_i,w_j) \sign([v_i]_q - [w_{j}]_q) - c_q(v_i,v_j) \sign([v_i]_q- [v_{j}]_q) \right)
\end{align} 
where 
\begin{align}
    c_q(v,w) = \frac{|[v]_q - [w]_q|}{\sqrt{([v]_q - [w]_q)^2 + \beta([v]_1 - [w]_1)^2 }}
\end{align}
For $\beta = 4n^2/\Delta^2$ and $\epsilon_1<\Delta/2$, we have 
\begin{align}
     c_q(v,w) & \geq \frac{|[v]_q - [w]_q|}{|[v]_q - [w]_q| + \sqrt{\beta}|[v]_1 - [w]_1|} \\
     & \geq |[v]_q - [w]_q|(1-\sqrt{\beta}|[v]_1 - [w]_1| ) 
\end{align}
Combining the above inequality with the result of Eq.~\eqref{eq:optimality_1st} yields 
\begin{align}
    c_q(v,w) \geq (1-\epsilon_1 \beta)|[v]_q - [w]_q| \geq \frac{1}{2} | v_q - w_q| 
\end{align}
for $\epsilon_1 \leq 1/(2\beta)$. Using the above result, we get
\begin{align}
    c_q(v_i,w_{\sigma(i)}) \geq \frac{1}{2}| [v_i]_q - [w_{\sigma(i)}]_q | 
\end{align}
For $j\neq \sigma(i)$, the following upperbound holds 
\begin{align}
      c_q(v_i,w_{j}) & \leq \frac{1}{\sqrt{\beta}([v_i]_1 - [w_j]_q)} \\ 
      & \leq \frac{1}{\sqrt{\beta}([w_i]_1 - [w_j]_q - \epsilon_1)} \\ 
      & \leq \frac{2}{\sqrt{\beta} \Delta} \quad \quad \quad (\epsilon_1 \leq \Delta/4) \\ 
      & \leq \frac{1}{2n} \quad \quad \quad (\beta = (4n^2)/\Delta^2)
\end{align}
Similarly, we get 
\begin{align}
    c_q(v_i,v_j) &\leq  \frac{1}{\sqrt{\beta}([v_i]_1 - [v_j]_q)} \leq   \frac{1}{\sqrt{\beta}(|[w_i]_1 - [w_j]_q|-2\epsilon_1)} \leq \frac{1}{2n}
\end{align}
The above bounds allows us to approximate the partial derivative used in Algorithm~\ref{alg:recovery_2d} as 
\begin{align}
   \left| \frac{\partial \text{E}_{V_\alpha^q}}{[\partial v_i]_q} - c(v_i,w_{\sigma(i)})\sign([v_{i}]_q - [w_{\sigma(i)}]_q) \right|  \leq  \frac{(n-1)}{n^3}
\end{align}
Using the above inequality, we establish the convergence of $[v_i]_q$ to $[w_{\sigma(i)}]_q$: 
\begin{align}
    \left| [v_i^{(j+1)}]_q - [w_{\sigma(i)}^{(j+1)}]_q \right| \leq \begin{cases} (1-\frac{\gamma_2}{2n^3})\left| [v_i^{(j)}]_q - [w_{\sigma(i)}^{(j)}]_q \right| & \left| [v_i^{(j)}]_2 - [w_{\sigma(i)}^{(j)}]_2 \right|\geq 2\gamma_2/n^2 \\ 
    \frac{2\gamma_2}{n^2} & \text{otherwise}
    \end{cases}
\end{align}
Induction over $j$ concludes the proof. 

\end{proof}


\begin{itemize}
    \item What if $\theta_i \in [0,2\pi]$? Everything goes well just need to modify the proof a bit. 
    \item Gradient descent in non-polar coordinates: It is exactly the same in 2d.
    \item More precise proof for the corollary
    \item Extending the convergence result to $d$-dimensional cases an non-polar coordinates
    \item cleaning the write-up for Francis
\end{itemize}

 \section{Measurement Design}
 \subsection*{A novel recovery feature map}
 \eqref{eq:kernel_relu} is not the only kernel that guarantees the recovery of empirical measures. Consider the following kernel
 \begin{align}
     k'(w,w') = \left( \pi - \phi(w,w')\right)^2, \quad \phi(w,w') = \frac{\langle w, w' \rangle}{\|w\| \|w'\|}
 \end{align}
 Similar to \ref{eq:kernel_relu}, the above kernel also recovers the empirical measure as it is proven in the next lemma. 
 \begin{lemma}
$L_{k'}(\sum_{i=1}^n \delta_{v_i}/n)$ admits only one critical point with distinct $v_{i} \in S_{d-1}$.   
 \end{lemma}
\noindent Given the above kernel, one can design a proper activation function $\varphi$ and measurements for the recovery of empirical distribution. Suppose $\Phi(\mu_n)$ represents non-linear measurements of a neural networks with a step activation function; then, $(\Phi(\mu))^{\otimes 2}$ is the feature map that produces $k'$. 

\subsection*{ReLU networks}
A popular choice of non-linear function $\varphi$ is ReLU function, i.e. $\varphi(a) = \max(0,a)$. Given $x_1 \dots x_n$ are drawn uniformly from unit sphere, then 
\begin{align}
    (2\pi d) K(w,w') = (\pi - \phi(w,w'))\cos(\phi(w,w')) + \sin(\phi(w,w'))
\end{align}
Here we show that $K$ is similar to $k'$ in gradient flow. 

\subsection*{Gradient flow in 2D}


 \subsection*{A note on convexity}
 Even if $n=2$ and $d=2$, $L$ is not convex with respect to parameters $v_1$ and $v_2$. \textcolor{red}{Illustrate this with some experiments!} 
 
 
 
 
 
 \section{Measurements}
So far, our results results rely on $x$ drawn uniformly from the unit sphere. Now, we study the role of the distribution of $x$ in the measure recovery. 

\subsection{A warm-up example}
Suppose that $x = (\sin(r),\cos(r))$ where $r \in [0,2\pi]$ is a random variable with law $p(r) = |\sin(r)|/4$. It seems that this law will break the recovery as its density is rather low around the zero. But, we observe that gradient descent easily recovers the sparse measure. Let us analytically justify this observation. The adjusted kernel with law of $x$(/$r$) makes the following closed from
\begin{align}
     k(w,v) = \E \left[ \varphi(x^\top v) \varphi(x^\top w) \right]  & = \E \left[ \varphi(\cos(\theta - r)) \varphi(\cos(\omega - r))  \right]\\ 
     & = \left( \left( \int_{0}^{a} + \int_{b}^{2 \pi}\right) dp(r) \right)
\end{align}
where $a = \pi/2 + \min\{ \theta, \omega\}$ and $b=3\pi/2 + \max\{ \theta, \omega\}$. Therefore 
\begin{align} \label{eq:sinkernel}
    k(\theta,\omega) = \frac{1}{2} - \frac{1}{4}\left|\sin(\theta) - \sin(\omega)\right|
\end{align}
Then, we can use change of variables as $\theta' = \sin(\theta)$ and $\omega'=\sin(\omega)$. We know that $L_\varphi$ admits a unique critical point with respect to $\theta'$. Since $\sin$ is monotone on $\theta \in (0, \pi/2)$, I conclude $L_\varphi$ also admits a unique critical point (with distinct particles) with respect to $\theta$. Next Corollary establishes the convergence of gradient flow. 
\begin{corollary}
Suppose  $d\theta_k/dt = -\nabla_{\theta_k} L_\varphi(\theta(t))$ holds. Define $\theta'_k(t) = \sin(\theta_k(t))$, and $\omega'_k = \sin(\omega_k)$. Let $\mu'$ and $\nu'(t)$ be sparse measures of particles $\{\theta'_k(t)\}$, and $\{\omega'_k\}$. Assuming that $\omega'_k, \theta'_k(0) \in (0,\pi/2)$ are distinct, then 
\begin{align}
     d W_1(\nu'(t),\mu'(t))/dt<0 ,\quad \text{and} \quad \theta'_k(t) \in (0,\pi/2)
\end{align}
for $\nu'(t) \neq \mu(t)$ as long as .
\end{corollary}
\begin{proof}
A straightforward application of chain rule yields:
 \begin{align} \label{eq:partial}
        d\theta'_k/dt &= - \frac{\partial L_\varphi }{\partial\theta_k}\left( \partial \theta'_k/ \partial \theta_k\right)  = - \left( \partial \theta'_k/ \partial \theta_k\right)^2 \frac{\partial L_\varphi }{\partial\theta'_k} 
 \end{align}
 Therefore
 \begin{align}
      d W_1/dt  \leq \frac{1}{n}\sum_{k=1}^n \sign\left(\theta'_k(t) - \omega'_{k}\right) d\theta'_k/dt 
\end{align}
By Eq.~\eqref{eq:partial}, we get
\begin{align}
     \sign\left(\theta'_k(t) - \omega'_{k}\right) d\theta'_k/dt  =  \underbrace{-\sign\left(\theta'_k(t) - \omega'_{k}\right) \frac{\partial L_\varphi }{\partial\theta'_k}}_{< 0 (Eq.\eqref{eq:flow_gaurantee})} \left( \partial \theta'_k/ \partial \theta_k\right)^2 < 0
\end{align}

\end{proof}
\subsection{Generalization}
Suppose the law of $x = (\sin(r),\cos(r))$ where $r$ is a random variable with pdf $p$ obeying: 
\begin{itemize}
    \item[i] $p(r+\pi/2) = p(r+3\pi/2)$. 
    \item[ii] $p(r)$ is absolutely continuous with respect to Lebesgue measure on $[0,2\pi]$.
\end{itemize}
Let $P$ be the cdf of $r$. Then, we get 
\begin{align} \label{eq:kernelp}
     k(\theta,\omega) = \text{constant} - \text{constant}\left|P(\theta) - P(\omega)\right|
\end{align}
holds for monotone $P:[0,0.5\pi)\to [0,1/4]$. Then, we can use the same argument in the previous section and prove the convergence of gradient descent. Therefore, we have now a class of kernels that guarantees the exact recovery of the sparse measure.
\subsection{Kernel construction}
So far, we have proven the recovery by \ref{eq:kernel_step} and also kernels in Eq.~\eqref{eq:kernelp}, and \eqref{eq:sinkernel}.  It is easy to check that the recovery of all kernels in the following form is guaranteed
\begin{align}
    k(\theta, \omega) = \sum_{i=1}^M \alpha_i \left( k_i(\theta,\omega) \right), \quad k_i(\theta,\omega) = \text{constant} - \text{constant} | f_i(\theta) - f_i(\omega) | 
\end{align}
for positive constants $\alpha_i$, and monotone functions $f_i: (0,\pi/2) \to \R$.
We also observed that the following kernels obtained from ReLU measurements
\begin{align}
    k(\theta,\omega) = (\pi - |\theta-\omega|)\cos(\theta-\omega) + \sin(\theta-\omega)
\end{align}
\textcolor{red}{Is it possible to construct a rich family of kernels including the above kernel with guaranteed convergence?}
To answer this question, I want to iteratively enlarge the set of kernel for which we have guaranteed convergence. For example, I observed that GD converges to $\mu$ with the following kernel
\begin{align}
    k(\omega,\theta) = (\pi - |\theta-\omega|)^2
\end{align}
For the above kernel 
\begin{align}
    k(\theta,\omega) = (\pi - |\theta-\omega|)^2
\end{align}
We observed the above kernel also recovers the sparse measure. But, why? 
We have 
\begin{align}
    \frac{\partial L_{\varphi'}}{\partial \theta_i } = \sum_{j} (\pi - |\theta_i - \omega_j|)\sign(\theta_i - \omega_j) - \sum_{j\neq i} (\pi - |\theta_i - \theta_j|)\sign(\theta_i - \theta_j)
\end{align}
\begin{align}
    \frac{\partial L_{\varphi'}}{\partial \theta_i } - \frac{\partial L_{\varphi'}}{\partial \theta_{i-1} } = \left( | \{ \omega_j >\theta_i\}|- | \{ \omega_j <\theta_i\} |  + (n-2i) -1 \right)| \theta_i - \theta_j| 
\end{align}
which is zero if $\theta_i = \omega_j$ assuming $\theta_i \neq \omega_j$.

\section{Reconstruction from finite measurements}
Since \ref{eq:kernel_step} is a shift-invariant kernel, there are random variables $a$ and $b$ such that 
\begin{align} \label{eq:shiftinvaraint} \tag{shift invariant kernels}
    k(\theta, \omega) = \E \left[ \sin(\theta a +b ) \sin(\theta a + b) \right] 
\end{align}
holds true. This allows us to draw a finite number of samples and theoretically study the recovery of sparse measure. Yet, this does not lead to a practical algorithm for the sparse measure recovery. 
\subsection{A search over shift-invariant kernels}

\section{Recovery from finite moments}
Algorithm~\ref{eq:gd_lp} requires the exact integration with respect to measure $p$. In neural network applications, we are often given a finite set of indices $\{s(\alpha_1), \dots, s(\alpha_m)\}$ where $\alpha_i$ are drawn i.i.d. from $p$. In this section, we develop a recovery algorithm from the finite random indices. The propose algorithm is based on the uniform-kernel estimation of $p$ as  
\begin{align}
    p_{m,h}(\alpha) = \frac{1}{2 m h} \sum_{i=1}^m \underbrace{K\left(\frac{ \alpha -\alpha_i}{h}\right)}_{p_i(\alpha)}, \quad K(x) = \delta_{x \in [-1,1]}.
\end{align}
Using the above smoothing of the empirical distribution, we can optimize the recovery objective with the analytical integration with respect to $p$, required for Algorithm~\ref{eq:gd_lp}. Define \begin{align}
    P_i(\alpha) = \int_0^\alpha p_i(\alpha') d\alpha' = \begin{cases} 
     \frac{\alpha-\alpha_i}{2h} &  \alpha - \alpha_i \in [-h, h] \\ 
     1 & \alpha - \alpha_i \geq h \\ 
     0 & \alpha - \alpha_i \leq -h
    \end{cases}
\end{align}
Invoking Prop.~\ref{prop:kernelp}, we get 
\begin{align*}
    \left( 2 n^2 m^2 h^2 \right)L_{m,h}(\theta) = \sum_{i,j=1}^n \sum_{p,q=1}^m 2\left( | P_q(\theta_i) - P_m(\omega_j)| - | P_q(\omega_i) - P_m(\omega_j)| - | P_q(\theta_i) - P_m(\theta_j)| \right) 
\end{align*}
The derivative $dL_{m,h}/(d\theta)$ only depends on the finite indices, so computable even if $p$ is unknown. If $p_{m,h}$ obeys Assumption~\ref{assumption}($\beta,B$), then Lemma~\ref{lemma:gdlp_convergence} establishes the polynomial-time complexity for the recovery. The next corollary determines $m$, $h$ and the total complexity of the recovery. 
\begin{corollary}
Suppose $p$ is $\Omega$-holder and obeys \ref{assumption}($\beta,B$); then, it is possible to recover $\mu_n$ using a finite set of random indices $\{ \alpha_i \sim p \}_{i=1}^m$ in $\bigo(B n^2/(\beta^{6+4/\Omega}\epsilon))$ with $m= \bigo(\beta^{-2-2/\Omega})$, $h=\Theta(m^{-1/(2\Omega+2)})$ at least with a constant probability.
\end{corollary} 
\begin{proof}
 We can ensure \ref{assumption}.i by adding at most $4m$ samples to the given set of samples. Invoking Thm.~2 of ~\cite{jiang2017uniform}, we get $|p_{m,h}(\alpha)-p(\alpha)| \leq \bigo(m^{-\Omega/(2\Omega +2)})$ holds with the probability $1-1/m$. If $ m^{-\Omega/(2\Omega +2)}=\bigo(\beta/2)$, then $p_{m,h}$ obeys \ref{assumption}($\beta/2,2B$).    Hence, we can use the convergence result of \ref{eq:gd_lp} established in Lemma~\ref{lemma:gdlp_convergence} to get the polynomial-time complexity $\bigo(m^2 n^2/(\beta^{2}\epsilon))$. 
\end{proof}


\section{Recovery from finite moments}
\noindent To implement \ref{eq:gd_polar}, we require the following function\footnote{Given $g$, one can compute the gradient of $L_p$ in the polar coordinates used in $L_p$ by the change of variable as $v_1 = \sin(\theta)$.}
\begin{align}
     g(v) = \frac{1}{n}\sum_{i=1}^n \left(\frac{d k(v,w_i)}{dv_1}\right).
\end{align}
Therefore, the gradient descent relies on an infinite number of non-polynomial moments. Here, we prove that the recovery is possible using a finite number of random moments. Our results rely on the random feature representation of kernel that was pioneered by the seminal work~\cite{rahimi2007random}. The \ref{eq:kernel_step} is a dot product kernel which can be estimated by a random polynomial feature map~\cite{kar12}. This features are generated by Maclaurin expansion of $h(x) = 1 - \frac{1}{\pi}\arccos(x)$ as $h(x) = \sum_{i=0}^n \alpha_i x^i$ where it is known coefficients $\alpha_i$s are non-negative~\cite{kar12}. Given $\{\alpha_i\}$ and drawing integer $N_i$ with density $P(N_i=k) = 1/2^k$, \cite{kar12} proposes the following features: 
\begin{align}
     \Phi_i(v) = \sqrt{\alpha_{N_i} 2^{N_i}} \prod_{j=1}^{N_i} (R_j^\top v),
\end{align}
where $R_j \in \{1,-1 \}^2$ are i.i.d. Rademacher random variables. \cite{kar12} shows that $\E \left[ \Phi_i(w) \Phi_i(w') \right] = k(w,w')$. Invoking bounds from empirical process theory, we prove a finite set of random features provides an approximation for $g$. 
\begin{lemma}[Lemmas 3 and 7 of \cite{kar12}]

\begin{align} 
 dk(v,w)/dv_1= \E_z \left[ \langle d\Phi_1(v)/dv_1, \Phi_1(w')\rangle  \right].
\end{align}
\end{lemma}
\begin{proof}
 $\Delta (v,w) = dk(v,w)/dv_1 - d\Phi_1(v)/dv_1 \Phi_1(w')$.
 \begin{align}
     d\Phi_1(v)/dv_1 P_1(w') = \sqrt{\alpha_{N} 2^{N}}\sum_{k=1}^n \prod_{j\neq k} (R_j^\top v)  [R_k]_1
 \end{align}
 \begin{align}
     \nabla_v d\Phi_1(v)/dv_1 P_1(w') = d\Phi_1(v)/dv_1 P_1(w') \left( \sum_{j=1}^{N} \left(1-[R_j]_1/(R_j^\top v)\right)R_j/((R_j^\top v)) \right) 
 \end{align}
 \begin{align}
      \| \nabla_v \Delta(v,w) \| \leq  \| \nabla_v (dk(v,w)/dv_1) \| +  \| \nabla_v \Phi_1(v)/dv_1 P_1(w') \|
 \end{align}
 \begin{align}
       \| \nabla_v \Phi_1(v)/dv_1 P_1(w') \Phi_1(w') \| \leq \alpha_N 2^N  
 \end{align}
\end{proof}


\noindent  Although $\xi_j$ may be unbounded, the expected value of $\max_j \xi_j$ is $\bigo(m)$. This obtains the average time complexity $\bigo(m^2)$ for the construction of the feature map, and $\bigo(m^3)$ to compute its derivative. 
\begin{theorem}
  Consider the feature map $\Phi(w) \in \R^m$ defined in the last lemma. Using $m=\bigo(n^4/\epsilon^2)$
\end{theorem}
\begin{proof}
\begin{align}
      \left| \theta_i^{(k+1)} - \omega_i \right|= \left|\theta_i^{(k)} - \omega_i  - \gamma \frac{d L}{d\theta_i} \mid_{\nu_n(k)} + \text{error}\right|.
  \end{align}
Suppose error$=\bigo(\gamma/(n^2\pi))$; then, we get 
\begin{align}
  W(\nu_n(k+1),\mu_n) 
     & \leq \begin{cases} 
      \max\{W(\nu_n(k),\mu_n) - \frac{\gamma}{n^2\pi},2\gamma\} & W(\nu_n(k),\mu_n)  \geq 2\gamma  \\ 
      2\gamma  & \text{otherwise} 
     \end{cases} \label{eq:convergencebound_gd}.
\end{align}
The same contradiction as Lemma~\ref{lemma:gd_convergence}.
\end{proof}


\subsection{Gradient flow} Ordinary differential equations (ODE) modeling first-order optimization methods have provided profound insights into the mechanisms of these methods. For example, ODEs convey the essence of acceleration for descent methods with momentum~\cite{su2014differential,zhang2021revisiting,zhang2021rethinking}. The ODE model of gradient descent globally converges when optimizing infinite-width neural networks~\cite{chizat2018global}. Inspired by these studies, we also analyze an ODE model of the gradient descent for neural moment matching, namely the following iterative algorithm:
\begin{align} \label{eq:gradient_flow} \tag{P-ODE}
   \frac{d\theta_i}{dt} & = - \frac{d L}{d \theta_i}\mid_{\nu_t} = \frac{1}{ \pi n^2} \left(\sum_{j\neq i, j=1}^n \text{sign}(\theta_i(t) - \theta_j(t)) -\sum_{j=1}^n \text{sign}(\theta_i(t) - \omega_j) \right),
\end{align}
where $\nu_t(w) = \frac{1}{n} \sum_{i=1}^n \delta_w(\theta_i)$.
We first study the convergence properties of the above ODE, then construct a recovery algorithm by integrating the ODE. This two-step approach allows us to study the convergence of gradient descent in a more principled way. The next lemma proves that $W(\nu_t,\mu)$ rapidly decreases with $t$.
\begin{lemma}[Convergence of \ref{eq:gradient_flow}]  \label{lemma:gradient_flow}
\ref{eq:gradient_flow} obeys
\begin{align}
     W(\nu_t,\mu) \leq \exp\left( -\left(\frac{1}{n
     \pi}\right)^2 t \right) W(\nu_0,\mu),
\end{align}
as long as all $\{\theta_i(0),\omega_i \in (-\pi,\pi)\}$ are distinct.
\end{lemma}

\begin{proof}
    Without loss of generality, we assume $\theta_1(t) \leq \dots \leq \theta_n(t)$ holds. For an infinitesimal $\Delta$, $\theta_1(t+\Delta),\dots,\theta_n(t+\Delta)$ may not be sorted. Yet, invoking Lemma~\ref{lemma:optimal_transport} yields:
    \begin{align} \label{eq:delta_argument}
        W(\nu_n(t+\Delta),\mu_n) - W(\nu_n(t),\mu_n) \leq -\sign(\theta_j(t)-\omega_j) \left( \frac{d L}{d \theta_j} \right) \Delta + o(\Delta),
    \end{align}
    for $j = \arg\max_{i}|\theta_i - \omega_i|$. Dividing both sides by $\Delta$ and taking the limit $\Delta \to 0$ obtains
    \begin{align} \label{eq:derivative_wass}
         \frac{d}{dt}\left(W(\nu_n(t),\mu_n) \right) \leq -\sign(\theta_j(t)-\omega_j) \left(\frac{d L}{d \theta_j}\right).
    \end{align}
    Plugging the bound of Lemma~\ref{lemma:gradient_dir} into the above inequality yields
    \begin{align}
 \frac{d}{dt}\left(W(\nu_n(t),\mu_n) \right) \leq -\frac{1}{\pi n^2}.
    \end{align}
     Since $ W(\nu_n(t),\mu_n) \leq \pi $,
    \begin{align}
        & \frac{d}{dt}\left(W(\nu_n(t),\mu_n) \right) \leq - \left(\frac{1}{\pi n}\right)^2 W(\nu_n(t),\mu_n)
        \\ \implies &  \frac{d}{dt}\left(W(\nu_n(t),\mu_n) \right) \left(W(\nu_n(t),\mu_n)\right)^{-1} \leq - \left(\frac{1}{\pi n}\right)^2.
    \end{align}
    The integration of the both sides over $t$ concludes the exponential convergence rate. 
\end{proof}


\subsection{Convergence of gradient flow}
We first study the convergence of gradient flow, namely the following ODE 
\begin{align} \label{eq:lode} \tag{$L_p$-ODE}
\frac{d \theta_i }{dt} =- \frac{d L_p}{d  \theta_i }\mid_{\nu_n(t)}.
\end{align}
Then, we establish a polynomial-time complexity for an algorithm obtained by the integration of the above ODE. Next lemma proves the above ODE contracts to $\mu_n$ with an exponential rate. 
\begin{lemma} \label{lemma:flow_lp}
Under \ref{assumption}.i, and \ref{assumption}.ii($\alpha$),  \ref{eq:lode} obeys 
\begin{align}
     W(\nu_n(t),\mu_n) \leq \exp\left( -\frac{\beta}{\pi n^2} t \right)  W(\nu_n(0),\mu_n) ,
\end{align}
as long as $\theta_i(0),\omega_i \in [0,\pi)$ are distinct.
\end{lemma} 
\noindent The proof is postponed to Appendix~\ref{sec:flow_lp}.

\subsection{Proof of Lemma~\ref{lemma:flow_lp}} \label{sec:flow_lp}

The proof is based on the change of variables as $\theta'_i(t) = P(\theta_i(t))$.
By the chain rule, we get
\begin{align} \label{eq:partial}
        \frac{d\theta_i}{dt} &= - \frac{d L_p}{d\theta'_i}\left( \frac{d \theta'_i}{ d \theta_i}\right)   = \left( - \frac{d L_p}{d\theta'_i}\right) p(\theta_i).
 \end{align}
 Without loss of generality, we assume $\theta_1(t) \leq \dots \leq \theta_n(t)$. Using Lemma~\ref{lemma:gradient_dir}, we get\footnote{Recall the derivation in Eq.~\ref{eq:delta_argument}}
  \begin{align} 
  \frac{d}{dt} \left( W(\nu_n(t),\mu_n) \right) & \leq  -\sign(\theta_j(t)-\omega_j) \left(\frac{d L_p}{d \theta_j}\right), \quad j = \arg\max_{i}|\theta_i - \omega_i| \\ 
  & \leq -\sign(\theta_j(t)-\omega_j) \left( \frac{d L_p}{d\theta'_j} p(\theta_j)\right).
   \end{align}
\noindent Since $P$ is a monotonically increasing function,  $\sign(\theta'_j(t) - \omega_j')  = \sign(\theta_j(t) - \omega_j)$ holds. Therefore, 
 \begin{align} 
  \frac{d}{dt} \left( W(\nu_n(t),\mu_n) \right) 
  & \leq - \left(\sign(\theta'_j(t)-\omega'_j)  \frac{d L_p}{d\theta'_j}\right) p(\theta_j) \\
  &  \leq - \beta \left(\sign(\theta'_j(t)-\omega'_j)  \frac{d L_p}{d\theta'_j}\right) \\ 
  & \leq -\frac{\beta}{n^2},
   \end{align}
   where we invoked Lemma~\ref{lemma:gradient_dir} to get the last inequality. Considering $W(\nu_n(t),\mu_n)\leq \pi $, we get
   \begin{align}
 \frac{d}{dt} \left( W(\nu_n(t),\mu_n) \right)/W(\nu_n(t),\mu_n) \leq -\frac{\beta}{n^2 \pi} .
   \end{align}
 Taking the integral of the both sides over $t$ concludes the proof.
 
 
 
 % \noindent
% \textbf{Independent vs. interacting particles}
%  How to reconstruct uniform measure over circle by moving particles?  We compare two models for moving particles: (i) a model of independent particles, (ii) a model of interacting particles. 
%  \begin{itemize}
%      \item[(i)] Billiard dynamics where particles are shot in random directions reflected from the boundary 
%      \item[(ii)] Interactive particles whose states are updated with interactions as 
%      \begin{align*} 
%      d w_i/dt = - \sum_{j\neq i} \nabla_{w_i} K( \|w_i - w_j\|), \quad K(a) = -\log(a) + a^2.
%      \end{align*}
%  \end{itemize}
%  Figure~\ref{fig:billiard} provides simulations for (i) and (ii). We observe (i) does not lead to a uniform distribution (proven by \cite{mather1984non}).
%  In (i) particles are independent, while while real particles may push or pull each other due to their magnetic spins. Model (ii) reseblems uniformly distributed particles by interactions between particles. Kernel $K$ in (ii) introduces forces between particles depending on their distance. Adapting the interaction kernel, one can construct uniform measure over ellipse~\cite{carrillo2022global} and high dimensional Torus~\cite{shu2021generalized}.  
% \input{billiard}

==> billiard.tex <==
\begin{figure}[t]

\begin{tabular}{c c}
      \begin{adjustbox}{valign=t}
      \begin{asy}[width=4cm,height=4cm]
import graph;

size(200);

// circle billiard
 path bill = Circle((0,0),90.0);
 real phi = 2*pi*0.23456;

// stadium billiard

draw(bill);


pair s = (20,20), db, dt = exp(I*phi), e = s+200*dt;
path traj = s--e;
real [] c;


for(int i=0; i<50; ++i) {

  c = intersect(bill, traj);
  e = point(traj, c[1]);
  db = dir(bill, c[0]);

  draw(s--e,red);
  dot(e,blue);

  dt = -dt + 2*dot(dt,db)*db;

  s = e;
  e = s + 200*dt;

  traj = (s+dt)--e;
}
\end{asy}
      \end{adjustbox}
      &  
      \begin{adjustbox}{valign=t}
      \begin{asy}[width=8cm,height=5cm]
import graph;

size(200);

// circle billiard
// path bill = Circle((0,0),90.0);
// real phi = 2*pi*0.23456;

// stadium billiard
path bill = (-50,-50)--(50,-50)--arc((50,0), 50, -90, 90)
  --(50,50)--(-50,50)--arc((-50,0), 50, 90, 270)--cycle;
real phi = 2*pi*0.123456;


draw(bill);


pair s = (20,20), db, dt = exp(I*phi), e = s+200*dt;
path traj = s--e;
real [] c;


for(int i=0; i<150; ++i) {

  c = intersect(bill, traj);
  e = point(traj, c[1]);
  db = dir(bill, c[0]);

  draw(s--e,red);
  dot(e,blue);

  dt = -dt + 2*dot(dt,db)*db;

  s = e;
  e = s + 200*dt;

  traj = (s+dt)--e;
}
\end{asy}
      \end{adjustbox}\\
\vspace{0.3cm}
   (i)  & (ii)
\end{tabular}
\caption{\footnotesize{\textbf{Billiard dynamics:}}}
\label{fig:billiard}
\end{figure}
